Revisiting Performance Claims for Chest X-Ray Models Using Clinical Context

Public datasets of Chest X-Rays (CXRs) have long been a popular benchmark for developing machine learning (ML) computer vision models in healthcare. However, the reported strong average-case performance of these models do not necessarily reflect their actual utility when used in heterogeneous clinical settings, potentially masking weaker performance in medically significant scenarios. In this work we use clinical context to provide a more holistic evaluation of models for CXR diagnosis. In particular, we use discharge summaries, recorded prior to each CXR, to derive a ``pre-CXR'' probability of each CXR label, as a proxy for existing contextual knowledge available to clinicians when interpreting CXRs. We use this measure to probe model performance along two dimensions: First, using a stratified analysis, we show that models tend to have lower performance (as measured by AUROC and other metrics) among individuals with higher pre-CXR probability. Second, by controlling for pre-CXR probability via matching and re-weighting, we demonstrate that performance degrades when the correlation is broken between prior context and the current CXR label, suggesting that model performance is highly sensitive to the underlying distribution of clinical context. Specifically, cases with high pre-test probabilities present a fundamentally more difficult visual classification task, highlighting a gap in clinical utility when models are applied to high-risk cohorts.

==> formatting.tex <==
% Formatting for notes
\addtolength{\oddsidemargin}{-1in}
\addtolength{\evensidemargin}{-1in}
\addtolength{\textwidth}{2in}

\hypersetup{
  colorlinks=true,
  linkcolor=RawSienna,
  citecolor=gray
}

\setlength{\parskip}{6pt}
\setlength{\parindent}{0pt}
\setlength{\headheight}{14pt}


==> packages.tex <==
% Get math tools and define theorems
\usepackage{lineno}
\usepackage{amssymb,amsmath,amsfonts,mathtools,dsfont,thmtools}

% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{conjecture}{Conjecture}[section]
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]
% \newtheorem{assumption}{Assumption}[section]
% \newtheorem{example}{Example}[section]
% \theoremstyle{remark}
% \newtheorem{remark}{Remark}[section]

% Normal Packages
\usepackage{csquotes}
\usepackage{comment}

\usepackage{tikz}
\usepackage{tikz-qtree}
\usetikzlibrary{bayesnet}

\usepackage{pgfplotstable}
\pgfplotsset{compat=1.18}

\usepackage{hyperref}
\usepackage[capitalize,noabbrev]{cleveref}

% Clever Ref Configuration, assuming capitalization above
\Crefname{assumption}{Assumption}{Assumptions}
\crefname{assumption}{Assumption}{Assumptions}


